CommRad: Context-Aware Sensing-Driven Millimeter-Wave Networks

Millimeter-wave (mmWave) technology is pivotal for next-generation wireless networks, enabling high-data-rate and low-latency applications such as autonomous vehicles and XR streaming. However, maintaining directional mmWave links in dynamic mobile environments is challenging due to mobility-induced disruptions and blockage. While effective, the current 5G NR beam training methods incur significant overhead and scalability issues in multi-user scenarios. To address this, we introduce CommRad, a sensing-driven solution incorporating a radar sensor at the base station to track mobile users and maintain directional beams even under blockages. While radar provides high-resolution object tracking, it suffers from a fundamental challenge of lack of context, i.e., it cannot discern which objects in the environment represent active users, reflectors, or blockers. To obtain this contextual awareness, CommRad unites wireless sensing capabilities of bi-static radio communication with the mono-static radar sensor, allowing radios to provide initial context to radar sensors. Subsequently, the radar aids in user tracking and sustains mobile links even in obstructed scenarios, resulting in robust and high-throughput directional connections for all mobile users at all times. We evaluate this collaborative radar-radio framework using a 28 GHz mmWave testbed integrated with a radar sensor in various indoor and outdoor scenarios, demonstrating a 2.5x improvement in median throughput compared to a non-collaborative baseline.

==> Makefile <==
TARGET           ?= main
TARGET_TYPE      ?= pdf
LATEXMK          ?= latexmk
LATEXDIFF        ?= latexdiff-vc

ifneq ($(V), 1)
Q                := @
LATEXMK_FLAGS    += -silent
else
Q                :=
LATEXDIFF_FLAGS  += -V
endif

UNAME_S          := $(shell uname -s)
TARGET_FILE       = $(TARGET).$(TARGET_TYPE)
TARGET_DIFF       = $(TARGET)-diff$(LATEXDIFF_BASE)

LATEXMK_FLAGS    += -$(TARGET_TYPE) -f

# Reference git branch/tag
LATEXDIFF_BASE   := submission2
LATEXDIFF_STYLE  := TRADITIONAL
# NOTE: vc-version does not take preamble
LATEXDIFF_FLAGS  += --git --flatten --force -r $(LATEXDIFF_BASE) 
LATEXDIFF_IGNORE := author,authornote,email,affiliation,institution,ccsdesc,renewcommand,section,subsecion,subsubsection
LATEXDIFF_NOENV  := (?:picture|DIFnomarkup|align|comment|CCSXML|thebibliography|figure|equation|tabular)[\w\d*@]*
LATEXDIFF_FLAGS  += --exclude-textcmd='$(LATEXDIFF_IGNORE)'

ifeq ($(shell which $(LATEXMK)), )
$(error "Please install `$(LATEXMK)`!")
endif
ifeq ($(shell which $(LATEXDIFF)), )
$(warning "Please install `latexdiff` or `latexdiff-vc` to use `make diff` function!")
endif

.PHONY: clean view check diff

$(TARGET_FILE): $(wildcard *.tex *.bib *.sty *.cls figures/*)
	@echo "Compiling..."
	$(Q) $(LATEXMK) $(LATEXMK_FLAGS) $(TARGET)

clean:
	@echo "Cleaning..."
	$(Q) $(LATEXMK) $(LATEXMK_FLAGS) $(TARGET) -C
	$(Q) rm -f $(TARGET).bbl $(TARGET_DIFF).bbl
	$(Q) if test -f $(TARGET_DIFF).tex; then $(LATEXMK) $(LATEXMK_FLAGS) $(TARGET_DIFF) -C; rm $(TARGET_DIFF).tex; fi

view: $(TARGET_FILE)
ifeq ($(OS), Windows_NT)
	$(Q) open $(TARGET_FILE)
else
ifeq ($(UNAME_S), Linux)
	$(Q) xdg-open $(TARGET_FILE) &
endif
ifeq ($(UNAME_S), Darwin)
	$(Q) open $(TARGET_FILE) &
endif
endif

check: $(TARGET_FILE)
	$(Q) grep -i -e "undefined" -e "multiply" $(TARGET).log || echo "Nothing found."

# NOTE: latexdiff will not work with IEEEtran style
diff: clean
	@echo "Compiling diff..."
	$(Q) $(LATEXDIFF) $(LATEXDIFF_FLAGS) $(TARGET).tex
	$(Q) $(LATEXMK) $(LATEXMK_FLAGS) $(TARGET_DIFF)


==> conclusion.tex <==
% \section{Conclusion}\label{sec:conclusion}
% % \vspace{-2mm}
% In this work, we present the first proactive beam management solution that optimizes both throughput and reliability in mmWave systems. We develop co-phasing, superresolution, and tracking algorithms to maintain multi-beam links based on low-overhead, standard compliant feedback. We evaluate the system on a testbed representative of 5G-NR PHY with 8x8 phased array and show reliability close to 1 and throughput gain of 1.5x. This work makes multi-beamforming a tractable for communication links and we believe that it paves the way for a new direction in mmWave where environmental reflections and careful channel estimation can improve beam management. Since multi-beams are a new class of beamforming itself, designing a robust networking system while multiplexing multiple users is an open challenge. 

\section{Acknowledgements}\label{sec:acks}

We are grateful to the anonymous reviewers and our shepherd, Prof.
Romit Roy Choudhury, for their insightful feedback. We thank Prof.
Gabriel Rebeiz, UCSD, and his group for the mmWave 5G
phased arrays and transceivers. The research is supported by NSF CCRI \# 1925767.

\noindent
% \textbf{Multi-user and MIMO setup.} MIMO helps in enhancing the diversity of single-user link, or it can enhance the multiplexing of multiple users. Prior work~\cite{jog2019many,ghasempour2018multi} has proposed interference-aware spatial multiplexing of beams in different directions for multiple users. \name can be combined with the above work to provide reliability to multiple clients at the same time and enable proactive tracking of multiple clients. In particular, some of the spatial beams can be used for enhancing the reliability of single-user while other beams can be used to improve the performance of multi-user.


% We plan to release our hardware setup related code to the broader community in the near future. 

%  \todo{In all our experiments, we fixed the total radiated power which reduces the EIRP of multi-beam compared to a single beam. In practice, multi-beam can be transmitted with higher power meeting the FCC regulation on EIRP and achieve even better performance.}
